Do We Need iPhone Moment or Xiaomi Moment for Robots? Design of Affordable Home Robots for Health Monitoring

In this paper, we study cost-effective home robot solutions which are designed for home health monitoring. The recent advancements in Artificial Intelligence (AI) have significantly advanced the capabilities of the robots, enabling them to better and efficiently understand and interact with their surroundings. The most common robots currently used in homes are toy robots and cleaning robots. While these are relatively affordable, their functionalities are very limited. On the other hand, humanoid and quadruped robots offer more sophisticated features and capabilities, albeit at a much higher cost. Another category is educational robots, which provide educators with the flexibility to attach various sensors and integrate different design methods with the integrated operating systems. However, the challenge still exists in bridging the gap between affordability and functionality. Our research aims to address this by exploring the potential of developing advanced yet affordable and accessible robots for home robots, aiming for health monitoring, by using edge computing techniques and taking advantage of existing computing resources for home robots, such as mobile phones.

==> Tex/backup.tex <==
\section{SYSTEM OVERVIEW}\label{sec:system}
A robot is composed of four parts: (1) a drive system: The drive system provides the necessary motion for the robot. It includes components like motors, wheels, tracks, or legs that allow the robot to move through its environment. 
% Whether it’s a wheeled robot cruising across a factory floor or a legged robot navigating rough terrain. 
(2) an actuator system: The actuator system translates electrical signals into physical movement. Actuators, e.g. servos, hydraulic cylinders, or pneumatic pistons, are responsible for executing specific tasks or actions which enable the robot to manipulate objects, lift weights, or perform precise movements. (3) a sensing system: The sensing system equips the robot with perception capabilities. Sensors gather information from and understand the surroundings environment. Common sensors include cameras, lidar, ultrasonic sensors, and infrared detectors. By processing sensory data, the robot can detect obstacles, measure distances, and recognise objects. (4) a control system: the control system acts as the brain of the robot. It processes input information from sensors, makes decisions, and generates output commands for the actuators. Microcontrollers, along with control algorithms, play a crucial role in controlling a robot. 
% Whether it’s maintaining balance, following a path, or responding to user commands, the control system ensures coordinated and purposeful actions.

\section{Edge Enabled Control System for Affordable Robots Design }\label{sec:method}
In this section, we will give a detailed design to reduce the cost of home robots.
Traditionally, robots carry their control systems onboard, often comprising powerful computing units, high-specification sensors to enable complex algorithms. However, the control system contributes majority of the overall cost, limiting the affordability of robotic solutions. To address this challenge and make the robots affordable, we move the control system from the robot side to the edge side and use our widely used mobile phone as the control system. Only cheap microcontrollers, along with communication modules, are kept and integrated into the robot to transfer data collected from sensors to the edge side. Specifically, we will make the following considerations:


\textbf{Mobile Phones as Control System:} These common mobile phones are equipped with powerful processors, sufficient memory, and communication capabilities. By repurposing these widely used mobile phones in the edge as control system of robots, we take advantage of their computational prowess without incurring additional costs. The specifically designed app or software interface on the phone becomes the gateway to controlling the robot.
The sensors in a robot still collect information about its surrounding environment. Instead of processing the data onboard, the robot transfers them to the edge side, i.e., the mobile phone in our context. Communication protocols, such as Wi-Fi, facilitate efficient data exchange for the further real-time decision making. 

\textbf{Edge Intelligence and Decision-Making:} The mobile phone's processing capabilities enable edge intelligence, which saving the cost. Algorithms running on the edge analyse sensor data, make decisions, and generate control signals to robots. For example, some some common operations are obstacle avoidance, path planning, or manipulation. Many mobile phones have dedicated neural processing unit to realise on-device inference for complicated machine learning models, such as Neural Engines in iPhone, Tensor processor in Google Pixel, etc.

\textbf{Minimalistic Robot Hardware:} To make the robot more affordable, we reduce its onboard components. Only cheap microcontrollers and essential communication modules are integrated directly into the robot to communication to the edger. The drive system, the actuator system and the sensing system are explicitly designed without adding extra unnecessary functions. By minimizing hardware complexity, we reduce manufacturing costs significantly.

\textbf{Affordability and Scalability:} The edge-enabled approach reduces the robot's upfront cost. Affordable microcontrollers and minimal onboard components keep manufacturing expenses low.


--------

% In the pursuit of creating cost-effective and accessible robots, a novel approach emerges: **edge-enabled control systems**. 
 

% To address this challenge, researchers and engineers are reimagining the control system's location. Instead of embedding it within the robot itself, they shift it to the **edge side**—a strategic move that leverages existing infrastructure and ubiquitous devices. Here's how it works:

1. **Mobile Phones as Control Hubs**:
   - The ubiquitous presence of smartphones provides a unique opportunity. These pocket-sized devices are equipped with powerful processors, ample memory, and versatile communication capabilities. By repurposing our widely used mobile phones as control hubs, we tap into their computational prowess without incurring additional costs. A simple app or software interface on the phone becomes the gateway to controlling the robot.

2. **Minimalistic Robot Hardware**:
   - To make the robot truly affordable, we strip down its onboard components. Only **cheap microcontrollers** and essential communication modules are integrated directly into the robot. These microcontrollers handle basic tasks such as sensor data acquisition, motor control, and communication with the edge hub. By minimizing hardware complexity, we reduce manufacturing costs significantly.

3. **Data Transfer to the Edge**:
   - The robot's sensors collect vital information about its environment—whether it's monitoring temperature, detecting obstacles, or measuring distances. Instead of processing this data onboard, the robot **transfers it to the edge side** (i.e., the mobile phone). This offloading minimizes the computational load on the robot itself.
   - Communication protocols like **Bluetooth**, **Wi-Fi**, or even **low-power cellular networks** facilitate seamless data exchange. The mobile phone acts as an intermediary, aggregating sensor inputs and relaying control commands back to the robot.

4. **Edge Intelligence and Decision-Making**:
   - The real magic happens at the edge. The mobile phone's processing capabilities enable **edge intelligence**. Algorithms running on the phone analyze sensor data, make informed decisions, and generate control signals. For instance, obstacle avoidance, path planning, or adaptive behavior can be computed right on the phone.
   - By leveraging the phone's existing ecosystem (including app development frameworks and community support), we unlock a wealth of possibilities. Machine learning models, rule-based logic, and even cloud-based services can enhance the robot's functionality without adding hardware complexity.

5. **Affordability and Scalability**:
   - The edge-enabled approach drastically reduces the robot's upfront cost. Affordable microcontrollers and minimal onboard components keep manufacturing expenses low.
   - Moreover, this paradigm scales effortlessly. As long as users have a compatible mobile phone, they can control multiple robots simultaneously. Whether it's a fleet of home cleaning bots or educational robots in a classroom, the edge hub remains consistent.

In summary, the edge-enabled control system revolutionizes robot design by democratizing access. By utilizing our everyday mobile devices as control hubs, we bridge the gap between affordability and functionality. As we envision a future where robots seamlessly collaborate with humans, this paradigm shift ensures that cutting-edge technology remains within reach for all, regardless of economic constraints.


This innovative approach not only makes robots more affordable but also empowers users to participate actively in the robotics ecosystem. As we embrace this edge-centric future, we pave the way for a new generation of accessible and intelligent robotic companions.


**Leveraging the Supply Chain for Affordable Robot Design**

In the pursuit of cost-effective robot design, the supply chain emerges as a critical enabler. By strategically optimizing supply chain processes, manufacturers can significantly reduce costs and enhance the affordability of robotic solutions. Here's how the supply chain plays a pivotal role:

1. **Strategic Sourcing and Procurement**:
   - **Component Cost Reduction**: Effective sourcing and procurement practices lead to cost savings. By negotiating favorable terms with suppliers, manufacturers secure components—such as **microcontrollers**, **communication modules**, and other essential parts—at competitive prices.
   - **Bulk Purchasing**: Leveraging economies of scale, manufacturers buy components in bulk. This reduces per-unit costs and ensures a steady supply of affordable materials.

2. **Lean Manufacturing and Just-in-Time (JIT) Production**:
   - **Efficient Production**: Implementing lean manufacturing principles minimizes waste, streamlines production, and reduces excess inventory. JIT production ensures that components arrive precisely when needed, avoiding unnecessary storage costs.
   - **Flexible Assembly**: A responsive supply chain allows manufacturers to adapt assembly lines quickly. When demand fluctuates, they adjust production volumes without overcommitting resources.

3. **Localization and Proximity to Suppliers**:
   - **Nearshoring**: Positioning manufacturing facilities closer to suppliers reduces transportation costs and lead times. By sourcing components locally or regionally, manufacturers avoid lengthy supply chains and associated expenses.
   - **Supplier Collaboration**: Collaborating closely with suppliers fosters innovation. Joint efforts to optimize designs, streamline logistics, and share cost-saving ideas benefit both parties.

4. **Supply Chain Resilience and Risk Mitigation**:
   - **Diversification**: Relying on a single supplier is risky. Diversifying sources ensures continuity even if one supplier faces disruptions. This resilience prevents costly production delays.
   - **Contingency Planning**: Preparedness for unexpected events—such as natural disasters, geopolitical shifts, or supply shortages—reduces vulnerability. Having backup suppliers or alternative components mitigates risks.

5. **Technological Advancements and Industry Collaboration**:
   - **Industry Consortia**: Collaborating within industry consortia fosters knowledge sharing. Manufacturers collectively address challenges related to affordability, standardization, and supply chain optimization.
   - **Technology Adoption**: Embracing emerging technologies—such as **robotic process automation (RPA)** for supply chain management—enhances efficiency. Automated inventory tracking, demand forecasting, and order fulfillment contribute to cost reduction.

6. **Lifecycle Cost Considerations**:
   - **Total Cost of Ownership (TCO)**: Beyond initial manufacturing costs, evaluating the entire lifecycle cost is crucial. Factors like maintenance, upgrades, and end-of-life disposal impact affordability. A well-managed supply chain ensures cost-effective operations throughout the robot's lifespan.

In summary, a resilient and agile supply chain is instrumental in making affordable robots a reality. By optimizing sourcing, production, and collaboration, manufacturers can create cost-efficient solutions that benefit both consumers and the industry at large 1234.

% Source: Conversation with Bing, 04/04/2024
% (1) Robots to the Rescue: Creating a Flexible Supply Chain. https://www.supplychainbrain.com/articles/38341-robots-to-the-rescue-creating-a-flexible-supply-chain.
% (2) Robots Boost Capability for Supply Chain Scalability. https://www.packagingtechtoday.com/machinery/robotics-automation/robots-boost-capability-for-supply-chain-scalability/.
% (3) Robots to the Rescue: Creating a Flexible Supply Chain. https://www.supplychainbrain.com/articles/38573-robots-to-the-rescue-creating-a-flexible-supply-chain.
% (4) 3 trends to watch as robots get faster, safer and better | Supply Chain .... https://www.supplychaindive.com/news/robotic-trends-faster-cheaper-productive-warehouse/518318/.
% (5) Automation and robotics: The supply chain of the future. https://supplychaindigital.com/technology/automation-and-robotics-supply-chain-future.

==> Tex/experiment.tex <==
\begin{figure}[!t]
\vspace{2mm}
	\centering
	\subfigure[Google Pixel 6 Mobile Phone]{
		\includegraphics[width=0.1\textwidth]{figure/hardware_phone_rotated.pdf}
		\label{fig:hardware_phone}
		}
		\subfigure[WiFi Access Points]{
		\includegraphics[width=0.2\textwidth]{figure/hardware.pdf}
		\label{fig:hardware_wifi}
		}


		\caption{Hardware: (a) Google Pixel 6 Mobile Phone carried by the user in the designed system. IMU measurements and WiFi RTT measurements are collected using this mobile phone for localisation purpose. }
		\label{fig:hardware}
		\vspace{-7mm}
\end{figure}

\begin{figure*}[!t]
% \vspace{2mm}
	\centering
	\subfigure[Ground Truth, {\color{green}{x}} shows WiFi access points] {
		\includegraphics[width=0.25\textwidth]{figure/d1/groundtruth_ap.pdf}
		\label{fig:traj_gt}
		}
        \subfigure[Trajectory Only Using IMU]{
		\includegraphics[width=.25\textwidth]{figure/d1/imu.jpg}
		\label{fig:traj_imu}
		}
        \subfigure[Trajectory with Traditional SLAM]{
		\includegraphics[width=.25\textwidth]{figure/d1/noslam.jpg}
		\label{fig:traj_noslam}
		}
  
        \subfigure[Trajectory Using SLAM with RSSI]{
		\includegraphics[width=0.25\textwidth]{figure/d1/rssi.jpg}
		\label{fig:traj_rssi}
		}
		\subfigure[Trajectory Using Proposed Method]{
		\includegraphics[width=0.25\textwidth]{figure/d1/proposed.jpg}
		\label{fig:traj_slam}
		}
  
  %           \subfigure[CDF of localisation errors]{
		% \includegraphics[width=.32\textwidth]{figure/d1/cdf.jpg}
		% \label{fig:cdf}
		% }

		\caption{Performances in Experiment 1:  (a) Ground Truth; (b) Trajectory Only Using IMU; (c) Trajectory with Traditional SLAM; (d) Trajectory Using Proposed Method; 
  % (e) CDF of localisation errors  
  }
		\label{fig:traj}
		\vspace{-7mm}
\end{figure*}


\begin{figure}[!t]
% \vspace{2mm}	
   \centering
    \includegraphics[width=.3\textwidth]{figure/d1/cdf.jpg}
    \caption{CDF of localisation errors in Experiment 1}\label{fig:cdf}
    \vspace{-7mm}
\end{figure}
\section{EVALUATION}\label{sec:exp}
In this section, we will show the details of the used hardware, performance metric and the evaluation of the proposed system in real environments. 
\subsection{Hardware}


Figure \ref{fig:hardware} shows the hardware used in the evaluation. We use one Google Nest WiFi router and three Google Nest WiFi points \cite{googlewifi} as the WiFi access points. The mobile device we use is Google Pixel 6. Other devices supporting IEEE 802.11mc can also be used for the same purpose. The full list of devices supporting IEEE 802.11mc can be found in \cite{android80211}. WiFi access points are deployed on one floor of a house.
% , the floor plan and the locations of the WiFi access points are shown in Figure XXX. 
There is no specific configuration for Google Nest WiFi routers and Nest WiFi points other than enabling WiFi RTT functions using the official Google WiFi App \cite{WifiRttScan}. For Google Pixel 6, the sampling rate of the IMU is set as 100 Hz, and the sampling rate of WiFi RTT is empirically set as 5 Hz. A higher sampling rate could be set in the mobile device, but that will lead to packet loss because of the burden of processing the ranging requests in the router end\footnote{One WiFi ranging measurement is averaged over a sequence of the ranging requests in the lower level layer, but the API to access each measurement is not available in the current Android Version Android 12 (version 8.4). }. 


\subsection{Performance Metric}
Our proposed system will focus on 2D localisation in the indoor environment.
In this section, we use the following metrics to evaluate the proposed indoor localisation system. 
 \begin{itemize}
     \item \textbf{Trajectories}: Trajectories using the proposed method, IMU based PDR and that using traditional SLAM \cite{Thrun05} as well as ground truth will be shown using figures, which will provide an intuitive image of the good performance of the proposed method. 
     \item \textbf{Root mean square of errors of the trajectory}: $RMSE =  \sqrt{  \Sigma^{i_e}_{i=i_s}{ e(i)^2 }/{(i_e-i_s)} } $, where $i_s$ and $i_e$ are the start point and end point of the whole trajectory, and $e(i)$ the error at the time point $i$. $e(i) = ||l(i) - g(t)||_2$, where $l(i)$ and $g(t)$ are estimated locations and ground truth in 2D, respectively. 
     \item \textbf{Cumulative distribution function (CDF) of localisation errors}: The CDF of localisation errors demonstrates the frequency that a localisation error is less than or equal to a corresponding error.
     \item \textbf{Localisation error of the end point}: As the proposed localisation method is based on the trajectory, a good quality localisation system should not have a huge cumulative error in the end.  

     
 \end{itemize}
 
We tested our proposed systems in two real environments within 10m$\times$5m and 20m$\times$35m areas, respectively.

\subsection{Experiment 1: Real Environment in a house} \label{subsec:exp1}
To evaluate the proposed system, the user walks on one floor in a house within 10 m$\times$5 m area. Figure \ref{fig:traj_gt} shows the ground truth of the trajectory. The situation is similar to walking in a house, where there is furniture, so that people can only walk in a certain area. The ground truth is obtained by manually labelled key points, such as turning points and adding loop closures to revised points, such as narrow corridors where people have to walk by.  

In this experiment, the total trajectory path is 308.8 m. Figure \ref{fig:traj_imu} shows the trajectory only using IMU. Compared with Figure \ref{fig:traj_gt}, there are two observations: (1) the shape of the trajectory is similar to the ground truth; (2) the trajectory has accumulative bias compared with the ground truth. This confirms that it is feasible to use an IMU based PDR method for the indoor localisation system, and a secondary mechanism, such as the loop closure method, is required to calibrate the raw trajectory. After considering WiFi RTT based loop closures, false positives are introduced, i.e., due to the noise and multipath effect, distant points could be clustered falsely for further loop closure. When using the traditional pose graph SLAM \cite{Thrun05}, as shown in Figure \ref{fig:traj_noslam}, it cannot provide accurate localisation performance. Different from traditional SLAM, the robust pose graph SLAM, as discussed, uses various weights for loop closures during the optimisation process, so the false positives of loop closures can be given less weight. Figure \ref{fig:traj_slam} shows the trajectory using the proposed method, which clearly shows its good performance and outperforms the IMU based PDR method. The trajectory in Figure \ref{fig:traj_slam} also confirms that the robust SLAM has the capability to handle the false positives of loop closures and obvious enhancement compared with the trajectory using traditional SLAM shown in Figure \ref{fig:traj_noslam}.

When looking at RMSE of the trajectory, the use of IMU PDR can achieve 2.67 m. When using traditional SLAM, the RMSE of the trajectory is 5.95 m. When using the proposed method, the RMSE of the trajectory can reach 0.13 m, which has significantly been increased compared with the use of IMU and traditional SLAM. 
The good performance of the proposed method can be further confirmed by the localisation error of the end point. When using IMU based PDR, the localisation error of the end point is 9.84 m. The use of the traditional SLAM and our proposed method can achieve nearly 0 m.
The good performance in this metric for the proposed method and traditional SLAM is due to loop closures near the end point. Although the use of traditional SLAM can achieve good performance in this metric, it can still be clearly seen in Figure \ref{fig:traj_noslam} that, for the most part of its estimate trajectory, the use of the traditional SLAM cannot achieve satisfactory localisation performance. 

Figure \ref{fig:cdf} shows the CDF of errors using different methods. It demonstrates that the 90th percentile tracking errors for the IMU based PDR, traditional SLAM and the proposed method are 9.12 m and 4.46 m, and 0.21 m, respectively. This means, when using the CDF of localisation errors as a metric, the proposed method can have 4242\% and 2023\% enhancement compared with the PDR and traditional SLAM, respectively.



\begin{figure*}[!t]
% \vspace{2mm}
	\centering
	\subfigure[Ground Truth. {\color{green}{x}} shows WiFi access points]{
		\includegraphics[width=0.18\textwidth]{figure/d6/groundtruth_ap.pdf}
		\label{fig:traj_gt:d6}
		}
        \subfigure[Trajectory Only Using IMU]{
		\includegraphics[width=.18\textwidth]{figure/d6/imu.jpg}
		\label{fig:traj_imu:d6}
		}
        \subfigure[Trajectory with Traditional SLAM]{
		\includegraphics[width=.18\textwidth]{figure/d6/noslam.jpg}
		\label{fig:traj_noslam:d6}
		}
            \subfigure[Trajectory with Traditional SLAM]{
		\includegraphics[width=.18\textwidth]{figure/d6/rssi.jpg}
		\label{fig:traj_rssi:d6}
		}
		\subfigure[Trajectory Using Proposed Method]{
		\includegraphics[width=0.18\textwidth]{figure/d6/proposed.jpg}
		\label{fig:traj_slam:d6}
		}
  
  %           \subfigure[CDF of localisation errors]{
		% \includegraphics[width=.32\textwidth]{figure/d6/cdf.jpg}
		% \label{fig:cdf:d6}
		% }

		\caption{Performances in a large area in Experiment 2:  (a) Ground Truth; (b) Trajectory Only Using IMU; (c) Trajectory with Traditional SLAM; (d) Trajectory Using Proposed Method; 
  % (e) CDF of localisation errors  
  }
		\label{fig:traj:d6}
		\vspace{-7mm}
\end{figure*}

\begin{figure}[!t]
% \vspace{2mm}	
   \centering
    \includegraphics[width=.3\textwidth]{figure/d6/cdf.jpg}
    \caption{CDF of localisation errors in Experiment 2}\label{fig:cdf:d6}
    \vspace{-7mm}
\end{figure}

\subsection{Experiment 2: Real Environment in a Large Area }


In this section, we evaluate the proposed system further in a much large environment within 20 m$\times$35 m area. The user walks on the same floor in the house in Section \ref{subsec:exp1}, as well as the nearby area including gardens and roads, and Figure \ref{fig:traj_gt:d6}, shows the ground truth of the trajectory with path length 236 m. In this experiment, the outdoor environment is used for a larger environment, we do not employ any measurements from GPS or other sensors for localisation purposes. The same observations as Experiment 1 can be found in Figures \ref{fig:traj_imu:d6} and \ref{fig:traj_noslam:d6}. IMU based estimate can achieve a reasonable trajectory but it is biased compared with the ground truth in Figure \ref{fig:traj_gt:d6}. Although loop closure constraints are considered in traditional SLAM, the noisy and ambiguous WiFi range measurements make the estimate trajectory inaccurate (see Figure \ref{fig:traj_noslam:d6}). Figure \ref{fig:traj_slam:d6} shows trajectory using the proposed methods, it is clearly seen that the proposed method can achieve a better performance compared with IMU only and traditional SLAM. When using the metric RMSE, our proposed method also shows significant improvement. The RMSE of the trajectory when using IMU PDR and traditional SLAM can achieve 2.11 m and 11.97 m, respectively. This confirms the fact seen in Figure \ref{fig:traj_noslam:d6} that the use of traditional SLAM does not enhance the localisation performance. When using the proposed method, the RMSE of the trajectory is 1.21m, which improves 74\% and 889\% compared with IMU based PDR and traditional SLAM, respectively. When using localisation error of the end point as the metric, the imu based method has a 2.52 m error. Both the proposed method and traditional SLAM achieve 1.21 m error, but it is clearly seen that the proposed method outperforms the traditional SLAM method in Figure \ref{fig:traj:d6}.



We also show the CDF of errors in Figure \ref{fig:cdf:d6}. It demonstrates that the 90th percentile tracking errors for the IMU based PDR, traditional SLAM and the proposed method are 4.10 m and 19.64 m, and 1.62 m, respectively. This means, when using the CDF of localisation errors as a metric, the proposed method can have 153\% and 1100\% enhancement compared with the PDR and traditional SLAM, respectively.


